HAMLET: Graph Transformer Neural Operator for Partial Differential Equations

We present a novel graph transformer framework, HAMLET, designed to address the challenges in solving partial differential equations (PDEs) using neural networks. The framework uses graph transformers with modular input encoders to directly incorporate differential equation information into the solution process. This modularity enhances parameter correspondence control, making HAMLET adaptable to PDEs of arbitrary geometries and varied input formats. Notably, HAMLET scales effectively with increasing data complexity and noise, showcasing its robustness. HAMLET is not just tailored to a single type of physical simulation, but can be applied across various domains. Moreover, it boosts model resilience and performance, especially in scenarios with limited data. We demonstrate, through extensive experiments, that our framework is capable of outperforming current techniques for PDEs.

==> Backups/Unboxing....tex <==
\subsection{Unboxing the \PhysGTN\ Architecture}

Our architecture comprises multiple learnable modules with diverse graph structures that collaborate to infer solutions on an evaluation graph. \PhysGTN\ can be used in three interrelated scenarios: 1) PDEs with multiple inputs, enabling accelerated solution processes, 2) incorporation of known underlying differential equations alongside data, and 3) utilisation of known data symmetries for network augmentation. \PhysGTN\  comprises an encoder and a decoder, which are detailed next.

\faHandPointRight[regular]  \textbf{\PhysGTN\ Encoder.}  The encoder's advantage lies in its divided input functionality. Multiple input streams can be used to handle systems with varying variables during the evaluation process, and a cross-attention mechanism can connect them. 
%
%We first formalise the concept of multiple inputs by defining the collection of sampling points as $D_i=\{x_k\}_{k=1}^{N_i}$ and assuming multiple different collection samples $i\in\{1, ..., n\}$, where $D_i\subset D,\forall i\in\mathbb{N}^+$. Each sampling has specific input features $\theta^{(i)}=\{\theta^{(i)}(x_k)\}_{k=1}^{N_i}$, which we write as $\theta^{(i)}(x_k)=\theta^{(i)}_k$. We define the evaluation point collection $D^{eval}=\{y_k\}_{k=1}^{N_{eval}}$, which corresponds to an additional discretisation of the input domain $D^{eval}\subset\mathcal{U}$. 
%
For each input module, we generate a unique graph $\mathcal{G}_i$ following the method in Section 3.1, resulting in double tuples $\{\mathcal{G}_i, D_i\}_{i=1}^n$ for the entire dataset. The encoder layers are equivalent for each input stream and use an additional positional encoding $\lambda_k$ to learn node positions. To encode nodes, we use a specific mechanism introduced in~\cite{kreuzer_rethinking_nodate} that efficiently uses only the first $m$ eigenvectors, similar to~\cite{dwivedi_generalization_2021}. We lift the node features $h_k$ and positional encodings $\lambda_k$ using lifting layers $\mathcal{L}$, which reads: $\tilde{h_i}=\mathcal{L}_1 h_i,\,  \tilde{\lambda_i} = \mathcal{L}_2\lambda_i,\,  \tilde{\tilde{h_i}}= \tilde{h_i} + \tilde{\lambda_i}$.
% \begin{equation}
%      \tilde{h_i}=\mathcal{L}_1 h_i\quad \;\; \tilde{\lambda_i} = \mathcal{L}_2\lambda_i  \;\;\;
%     \tilde{\tilde{h_i}}= \tilde{h_i} + \tilde{\lambda_i}
% \end{equation}
   
To handle the complexity of the tasks, we increase the dimension of the latent space $\mathrm{dim}V_2 > \mathrm{dim}V_1$, following a similar approach used in other PDE applications~\cite{brunton2020machine}. Once the feature vectors are lifted into the higher-dimensional space, we input the encoded latent vector into the transformer block $\mathcal{GT}$: $\hat{h}_i^{\ell+1} = \mathcal{GT}(\tilde{\tilde{h_i}}^{\ell})$. We repeat this procedure $L\in\mathbb{N}^+$  times, obtaining an output latent feature vector $\hat{h}_i^{L}$  for each node, denoted as $\hat{h}_i^{L}=\textbf{h}_i$ for simplicity. 

After completing the graph transformer cycle, each dataset sampling $D_i$ corresponding to a graph $\mathcal{G}_i$ will have a collection of finalised feature vectors $\{\textbf{h}^{(i)}_k\}_{k=1}^{N_i}$ with $N_i=|D_i|$. We assume that $N_i=N_j, \forall i,j$, and perform the cross-attention modules sequentially in a pyramid-structured manner on the $D_i$ datasets. If $n$ is even, we apply the cross-attention module to the modules with graphs  $(\mathcal{G}_{2j+1}, \mathcal{G}_{2j+2})$  where $j\leq (n-2)/2$. If $n$ is odd, we first apply the cross-attention modules to the $n-1$ elements, and then in the second iteration, we can apply the cross-attention on the $\mathcal{G}_{n-1/2}$ graph with $\mathcal{G}_n$. This procedure is repeated until $n=1$. The cross-attention is defined as:
\begin{equation}
z_j\left(h_{i^{\prime}}\right)=\sum_{l=1}^{N_b} \frac{\sum_{i=1}^{N_s} k_l\left(\textbf{h}^{(b)}_i\right) v_j\left(\textbf{h}^{(b)}_i\right)}{n} q_l\left(\textbf{h}^{(b)}_{i^{\prime}}\right).
\end{equation}
This process is repeated iteratively until a final collection of feature vectors $\{\textbf{h}^{(final)}_k\}_{k=1}^N$is obtained.


\faHandPointRight[regular]  \textbf{\PhysGTN\ Decoder.}  During evaluation, we can use other nodes $D_{eval}=\{h^{(eval}_j\}_{j=1}^{N_{eval}}$. The corresponding graph is passed through its encoder, and at the final layer, it is merged with the final feature vector. Evaluation can also be performed at other collocation points, where only positions are known. During the final cross-former attention step, all the information from the nodes at the evaluation point is combined:
%
\begin{equation}
\begin{split}
    &h^{(eval)^\prime}_j=z_j\left(h_{i^\prime}^{(eval)}\right)= \\
    &\sum_{l=1}^{N_{eval}} \Bigg[ \frac{\sum_{i=1}^{N_{final}} k_l\left(\textbf{h}^{(final)}_i\right) v_j\left(\textbf{h}^{(final)}_i\right)}{n}  q_l\left(\textbf{h}^{(eval)}_{j}\right) \Bigg].
\end{split}
\end{equation}
The set of node features  $\{h^{eval}_k\}_{k=1}^{N_{eval}}$ is then passed through a recurrent neural network with LayerNorm to obtain the network's evaluation at the respective time point:
\begin{equation}
\widehat{\textbf{h}}^{(eval)}_i = \left(\mathcal{F}(h^{(eval)}_j+h^{{(eval)}^\prime}_j))+ (h^{(eval)}_j+h^{{(eval)}^\prime}_j)\right)
\end{equation}
To consider the steady-state solution or analyse the dynamics over time, we lift our representation into a higher-dimensional space, increasing the degrees of freedom. However, tracking all problem parameters raises complexity. Instead, we adopt an autoregressive approach, propagating latent feature vectors using a recurrent architecture. This reduces model complexity~\cite{brandstetter2022message,li_transformer_2022,wu_learning_nodate}. Given the encoded node features  $\widehat{\textbf{h}}^{(eval)}_i$, we use a standard multilayer perceptron with a predefined time width discretisation $\delta t$. The discretisation determines the depth of the autoregressive model. Let $\mathcal{R}$ denote the recurrent layer. The propagation in the latent space is given by:
\begin{equation}
\widehat{\textbf{h}}^{(eval)}_{(i,t+\Delta t)} = \mathcal{R}\widehat{\textbf{h}}^{(eval)}_{i(t)} + \widehat{\textbf{h}}^{(eval)}_{(i,t+\Delta t)},
\end{equation}
after evolving the solution until the desired time $T$, we project it onto the required space using the projection layer $\mathcal{P}$: $u(x_i, T) = \textbf{h}^{(eval)}_{i,T} = \mathcal{P}\widehat{\textbf{h}}^{(eval)}_{(i, T)}$.

%% add the explicit definition on the PDE and data constraint cases  
% 

%%%%%%%%%%%%%%%
%%% comment on the loss used---
\faHandPointRight[regular]  \textbf{\PhysGTN\ Loss Function \& Discretisation Invariance.} 
We aim to learn the mapping between two infinite-dimensional spaces using a finite collection of dataset pairs. Our objective is to optimise the parameters $\mu\in\mathbb{R}^N$ to obtain the best possible approximation $\tilde{\mathcal{S}}_{\mu_{opt}}\sim \mathcal{S}$, which represents a specific configuration of the operator map. We can solve this problem by minimising the empirical risk considering an entire sampling set of $N$ independent and identically distributed (i.i.d.) data sets, which is given by:
%
\begin{equation}
\begin{split}
\min _{\mu \in \mathbb{R}^p}\mathcal{L}_{\text {data }}\left(u, \mathcal{S}_\mu(\theta)\right) &= \min _{\mu \in \mathbb{R}^p}\mathbb{E}_{\theta \sim \nu}
\left\|u-\mathcal{S}_\mu(\theta)\right\|_{\mathcal{V}}^2 \\
&\approx \min _{\mu \in \mathbb{R}^p} \frac{1}{N} \sum_{i=1}^N\left\|u^{(i)}-\mathcal{S}_\mu\left(\theta^{(i)}\right)\right\|_{\mathcal{V}}^2
\end{split}
\label{eq:TheoreticalLossDataOperator}
\end{equation}
%
Since the data pairs $\{\theta^{(i)},u^{(i)}\}_{k=1}^N$ are the discretisations of our continuous space. We assume we have only access to the pointwise evaluation of finite points. Let $\mathcal{U}^{(i)}=\{x_{k}^{(i)}\}_{k=1}^{L_i} \subset \mathcal{U}$ be a $L_i$-point discretisation of the domain $\mathcal{U}$. Despite being trained on a $L_i$-point discretisation, the operator $\tilde{S}_\mu$ should be able to provide $u(x)$ for any arbitrary $x \in \mathcal{U}$ given an input $\theta \in \mathcal{P}$. In particular, the discretised architecture maps into the space $\mathcal{V}$ and not into a discretisation thereof.

\Angie{the following part only if we have space otherwise to be moved to the supplementary:}
Suppose $\mathcal{P}$ is a Banach space of $\mathbb{R}^s$-valued functions on the domain $\mathcal{U} \subset \mathbb{R}^n$. Let $\mathcal{S}: \mathcal{U} \rightarrow \mathcal{V}$ be an operator, $\mathcal{U}_L$ be an $L$-point discretisation of $\mathcal{U}$, and $\tilde{\mathcal{S}}_\mu$ the approximate solution operator. For any compact $K \subset \mathcal{P}$, one can define the maximum offset of the operators following the ideas of Kovachki et al.~\cite{kovachki_neural_2022}:
\begin{equation}
\label{eq:MaximumOffset}
R_K\left(\mathcal{S}, \tilde{\mathcal{S}}_\mu, \mathcal{U}_L\right)=\sup _{\theta \in K}\left\|\hat{\mathcal{S}}\left(\mathcal{U}_L,\left.\theta\right|_{\mathcal{U}}\right)-\mathcal{S}(\theta)\right\|_{\mathcal{V}} 
\end{equation}
%
Given a set of discretisations $\{\mathcal{U}^{(i)}\}_{i=1}^{\infty}$ with the condition $\mathcal{U}^{(i)}\subset \mathcal{U}^{(j)}$ for $j>i$ of the domain $\mathcal{U} \subset \mathbb{R}^n$ such that $\mathcal{U} \subset\cup_{i=1}^{\infty} \mathcal{U}^{(i)}$, we say $\tilde{\mathcal{S}}_\mu$ is discretisation-invariant if the offset tends to zero when evaluating and training the neural operator $\tilde{\mathcal{S}}^{(i)}$ on other $N_i$ discretisations, for any $\theta \in \mathcal{P}$ and any compact set $K \subset \mathcal{P}$:
\begin{equation}
\label{eq:LimitMaximumOffset}
\lim _{N \rightarrow \infty} R_K\left(\mathcal{S}(\cdot, \theta), \tilde{\mathcal{S}}^{(N)}(\cdot, \cdot, \theta), \mathcal{U}^{(N)}\right)=0    
\end{equation}
To show that a neural network architecture is numerically discretisation-invariant, we must show that the approximation error is approximately constant as we refine the discretisation.

% \textit{Physics-Informed Loss.} To extend the framework to unsupervised and semi-supervised learning, we introduce a second approach metric that learns the operator based on the known parametric partial differential equation. The idea is to use the underlying PDE as a loss metric and find the parameters $\mu$ by minimising the physics-informed loss using automatic differentiation. In the case of stationary problems, the physics-informed loss is defined as the squared norm of $L^2(\mathcal{D})$. For one-instance learning and following previous notation, the loss function minimisation can be expressed as:
% %Note: add the multi-instance def
% \begin{equation}
% \label{eq:TheoreticalLossPDE}
% \begin{aligned}
% \min _{\mu \in \mathbb{R}^p}\mathcal{L}_{\mathrm{pde}}\left(a, \tilde{\mathcal{S}}_\mu(\theta)\right) & =\min _{\mu \in \mathbb{R}^p}\left\|\mathcal{L}_\theta\left( \tilde{\mathcal{S}}_\mu(\theta)\right)\right\|_{L^2(\mathcal{D})}^2 +\min _{\mu \in \mathbb{R}^p}\alpha\left\|\left.\tilde{\mathcal{S}}_\mu(\theta)\right|_{\partial\mathcal{D}}-u_b\right\|_{L^2(\partial \mathcal{D})}^2 \\
% & =\min _{\mu \in \mathbb{R}^p}\int_D\left|\left(\mathcal{L}_\theta(\tilde{\mathcal{S}}_\mu(\theta)(x)\right)\right|^2 \mathrm{~d} x+\min _{\mu \in \mathbb{R}^p}\alpha \int_{\partial D}\left|\tilde{\mathcal{S}}_\mu(\theta)(x)-u_b\right|^2 \mathrm{~d} x \\
% \end{aligned}
% \end{equation}
%\subsection{Understanding the Intricacies of the Loss Function for \PhysGTN}

%\Angie{---------------------------------------------------}

%\section{Architecture}

